HistoRAG: A Citation-Grounded Question Answering Assistant for Teaching with Scanned Local History and Heritage Archives

Teachers who prepare lessons on local history and cultural heritage work from material that is hard to use. The primary sources are scanned books without a text layer, and the supporting records are administrative catalogs released as spreadsheets. A general chatbot answers such questions fluently but without a verifiable source, which is the property a teacher needs most. This paper presents HistoRAG, a question answering assistant that answers from one regional collection and cites a volume and a page for every fact. HistoRAG transcribes each page with a vision language model and keeps a line level confidence from the token probabilities. It builds three stores from the same collection: a hybrid text index, a relational catalog database, and a knowledge graph extracted only from entity dense passages. A lightweight router sends each question to the stores it needs, so that counting questions reach the database and relational questions reach the graph. We build a benchmark of 516 questions over a collection of 36 scanned volumes and the heritage catalogs of the same region, covering statistical, factual, temporal, and multi-hop questions. HistoRAG answers more questions correctly than passage retrieval baselines and than a graph based retrieval system, at a far smaller cost per question. The assistant runs behind a chat interface, so a teacher can check any statement against the page it came from.

==> figs/fig1/panel_a.tex <==
% Panel (a): confidence-carrying transcription. Local frame 5.0 x 5.6.
% Exit ports: (aOutText) right edge of the line column, (aOutCat) catalog well.
% The confidence levels drawn below are schematic, not measured values.

\draw[hrpanel] (0,0) rectangle (5.0,5.6);
\node[hrtitle] at (0.18,5.30) {(a) Transcription};
\node[hrsub]   at (0.18,5.00) {scanned pages and catalogs};

% ---- scanned page ---------------------------------------------------
\draw[hrwell] (0.25,1.85) rectangle (1.65,4.65);
\foreach \y/\l in {4.38/1.10, 4.16/1.05, 3.94/1.10, 3.72/0.70,
                   3.30/1.10, 3.08/1.00, 2.86/1.10, 2.64/1.05, 2.42/0.85, 2.20/0.55}
  {\draw[hrtext] (0.42,\y) -- ++(\l,0);}
\node[hrlab, anchor=north] at (0.95,1.76) {page image};

% ---- vision language model -------------------------------------------
\draw[hrcard] (1.92,3.10) rectangle (2.66,3.70);
\node[hrlab] at (2.29,3.40) {VLM};
\draw[hrflow] (1.65,3.40) -- (1.92,3.40);
\draw[hrflow] (2.66,3.40) -- (2.92,3.40);

% ---- transcribed lines with confidence -------------------------------
\draw[hrwell] (2.92,2.20) rectangle (4.80,4.60);
\node[hrlab, anchor=south] at (3.55,4.64) {lines};
\node[hrlab, anchor=south] at (4.45,4.64) {$c(\ell)$};
\foreach \y/\l/\c in {4.30/0.98/0.97, 3.85/0.85/0.95, 3.40/0.95/0.62, 2.95/1.00/0.98, 2.50/0.70/0.94} {
  \ifdim\c pt<0.8pt
    \draw[draw=hrAmber, line width=1.1pt, line cap=round] (3.06,\y) -- ++(\l,0);
    \draw[hrhair, fill=white] (4.25,\y-0.06) rectangle (4.65,\y+0.06);
    \fill[hrAmber] (4.25,\y-0.06) rectangle ({4.25+0.40*\c},\y+0.06);
  \else
    \draw[hrtext] (3.06,\y) -- ++(\l,0);
    \draw[hrhair, fill=white] (4.25,\y-0.06) rectangle (4.65,\y+0.06);
    \fill[hrSlate] (4.25,\y-0.06) rectangle ({4.25+0.40*\c},\y+0.06);
  \fi
}
\node[hrchipA, anchor=north] at (3.86,2.10) {low-confidence line};

% ---- heritage catalogs ----------------------------------------------
\draw[hrwell] (0.25,0.55) rectangle (1.65,1.35);
\foreach \y in {0.75,0.95,1.15} {\draw[hrhair] (0.25,\y) -- (1.65,\y);}
\foreach \x in {0.62,1.08} {\draw[hrhair] (\x,0.55) -- (\x,1.35);}
\node[hrlab, anchor=north] at (0.95,0.46) {heritage catalogs};

\coordinate (aOutText) at (4.80,3.40);
\coordinate (aOutCat)  at (1.65,0.95);


==> figs/fig1/panel_b.tex <==
% Panel (b): three offline stores. Local frame 5.6 x 5.6.
% Card centres sit at y = 4.25 / 2.75 / 0.95 so that the connectors to
% panel (c) and the catalog connector from panel (a) are straight by construction.
% Entry ports (bIn1..3) on the left card edges, exit ports (bOut1..3) on the right.

\draw[hrpanel] (0,0) rectangle (5.6,5.6);
\node[hrtitle] at (0.18,5.30) {(b) Offline stores};
\node[hrsub]   at (0.18,5.00) {one collection, three views};

% ---- text index ------------------------------------------------------
\draw[hrcardB] (0.90,3.70) rectangle (5.35,4.80);
\node[hrhead, text=hrBlue!72!black] at (1.05,4.53) {Text index};
\node[hrchipN, anchor=west] (bDense) at (1.05,4.02) {dense};
\node[hrchipN, anchor=west] (bBm25)  at ([xshift=2pt]bDense.east) {BM25};
\node[hrchipA, anchor=west]          at ([xshift=2pt]bBm25.east) {confidence weighting};

% ---- knowledge graph -------------------------------------------------
\draw[hrcardP] (0.90,2.05) rectangle (5.35,3.45);
\node[hrhead, text=hrPlum!72!black] at (1.05,3.18) {Knowledge graph};
\node[hrchipN, anchor=west] at (1.05,2.72) {top-$\rho$ chunks by $d(x)$};
\node[hrchipA, anchor=west] at (1.05,2.34) {confidence-gated merge};
\begin{scope}[hrPlum]
  \coordinate (g1) at (4.30,3.02);
  \coordinate (g2) at (4.88,3.12);
  \coordinate (g3) at (4.62,2.62);
  \coordinate (g4) at (5.12,2.40);
  \coordinate (g5) at (4.18,2.40);
  \draw[line width=0.45pt] (g1) -- (g2) -- (g3) -- (g1) (g3) -- (g4) (g3) -- (g5);
  \foreach \p in {g1,g2,g3,g4,g5} {\filldraw[fill=white, line width=0.5pt] (\p) circle (1.8pt);}
\end{scope}

% ---- catalog database ------------------------------------------------
\draw[hrcardG] (0.90,0.45) rectangle (5.35,1.45);
\node[hrhead, text=hrGreen!62!black] at (1.05,1.19) {Catalog database};
\node[hrchipN, anchor=west] (bSites)  at (1.05,0.74) {sites};
\node[hrchipN, anchor=west] (bRelics) at ([xshift=2pt]bSites.east) {relics};
\node[hrchipN, anchor=west]           at ([xshift=2pt]bRelics.east) {survey};
\begin{scope}[hrGreen]
  \draw[line width=0.45pt, fill=white] (4.40,0.62) rectangle (5.18,1.28);
  \fill[hrGreenF] (4.40,1.10) rectangle (5.18,1.28);
  \foreach \y in {0.84,0.97,1.10} {\draw[line width=0.3pt] (4.40,\y) -- (5.18,\y);}
  \foreach \x in {4.66,4.92} {\draw[line width=0.3pt] (\x,0.62) -- (\x,1.28);}
\end{scope}

\coordinate (bIn1)  at (0.90,4.25);
\coordinate (bIn2)  at (0.90,2.75);
\coordinate (bIn3)  at (0.90,0.95);
\coordinate (bOut1) at (5.35,4.25);
\coordinate (bOut2) at (5.35,2.75);
\coordinate (bOut3) at (5.35,0.95);


==> figs/fig1/panel_c.tex <==
% Panel (c): routed question answering. Local frame 5.2 x 5.6.
% Evidence chips share the y of the store cards in panel (b): 4.25 / 2.75 / 0.95.
% Entry ports (cIn1..3) are the chips' west anchors.

\draw[hrpanel] (0,0) rectangle (5.2,5.6);
\node[hrtitle] at (0.18,5.30) {(c) Online answering};
\node[hrsub]   at (0.18,5.00) {routing and grounded generation};

% ---- evidence from the routed stores ---------------------------------
\node[hrchipB, anchor=west] (cT) at (0.30,4.25) {passages};
\node[hrchipP, anchor=west] (cK) at (0.30,2.75) {relations};
\node[hrchipG, anchor=west] (cS) at (0.30,0.95) {SQL rows};
\coordinate (cIn1) at (cT.west);
\coordinate (cIn2) at (cK.west);
\coordinate (cIn3) at (cS.west);

% ---- question, router, generator, answer ----------------------------
\node[hrcard, align=left, text width=2.75cm, inner sep=3pt, font=\hrtiny] (cQ) at (3.55,4.25)
  {Q: Which heritage sites in this city hold the highest protection level?};
\node[hrcard, align=center, text width=2.75cm, inner sep=3pt, font=\hrtiny] (cR) at (3.55,3.35)
  {router selects $R \subseteq \{\mathrm{sql}, \mathrm{kg}, \mathrm{text}\}$};
\node[hrcard, align=center, text width=2.75cm, inner sep=3pt, font=\hrtiny] (cG) at (3.55,1.95)
  {grounded generation};
\node[hrwell, align=left, text width=2.75cm, inner sep=3pt, font=\hrtiny] (cA) at (3.55,0.90)
  {answer with citations\\ $[1]$ volume, page\\ $[2]$ catalog};

\draw[hrflow] (cQ.south) -- (cR.north);
\draw[hrflow] (cG.south) -- (cA.north);

% evidence bus: every chip joins one vertical line, which feeds the generator
\coordinate (cbus) at (1.95,0);
\draw[hrbus] (cT.east) -- (cT.east -| cbus);
\draw[hrbus] (cK.east) -- (cK.east -| cbus);
\draw[hrbus] (cS.east) -- (cS.east -| cbus);
\draw[hrbus] (cT.east -| cbus) -- (cS.east -| cbus);
\draw[hrflow] (cG.west -| cbus) -- (cG.west);
\fill[hrSlate] (cG.west -| cbus) circle (1.15pt);

% the router gates which stores are queried
\draw[hrsel] (cR.west) -- (cR.west -| cbus);
\fill[hrSlate] (cR.west -| cbus) circle (1.15pt);

